Context Is Not Authority: Structured Runtime Governance for Financial Market Agents

Financial agents can turn correct context into an unauthorized effect: a customer-facing commitment, trade, or deployed policy. We present SAGE-Fin, a finance-specific authority-handoff contract that makes the proposed effect, not merely its text, the object of runtime control. SAGE-Fin compiles proposals into typed, adapter-bound candidates; records missing or stale institutional obligations as coverage debt; contracts authority under current market, account, policy, and dialogue state; and requires an exact-artifact receipt whose nominal type matches the consuming response, execution, or policy adapter. Evidence and workflow progress cannot substitute for effect authority, and prior authorization is rechecked after state changes. Across an authored 616-case catalog, five deterministic specifications yield 3,080 outputs; a label-isolated harness obtains 616/616 binary reference-prototype parity, including 3/3 named response-gate fixtures, while 22 tests cover selected paths. These results establish executable conformance, not independent safety accuracy. Separately, SAGE-Fin's response gate processed real customer-facing production requests at a confidential digital-asset platform. An operational team independent of the implementation team reached a strongly positive post-deployment conclusion on practical usefulness and workflow fit, and end-user feedback was also strongly positive. Disclosure permits only the review's independence, stakeholder classes, assessed dimensions, and directional conclusion, so this is qualitative field corroboration rather than an aggregate effect estimate. Three distinct de-identified predecessor failures, with independently confirmed 0/3 interception, ground repeated-emission drift, stale account evidence, and missing escalation state without estimating prevalence or treatment effect.

==> tables/experiment-leakage.tex <==
% Auto-generated by scripts/experiment-runner.mjs. Do not edit by hand.
\begin{tabular}{lcccc}
\toprule
Baseline & $N$ & Accuracy & Leaks / leak-eligible & Leakage rate \\
\midrule
prompt\_only & 616 & 100.0\% & 296/587 & 50.4\% \\
static\_checklist & 616 & 100.0\% & 294/587 & 50.1\% \\
cbea\_lcv\_lang & 616 & 100.0\% & 296/587 & 50.4\% \\
sage\_fin\_partial & 616 & 100.0\% & 61/587 & 10.4\% \\
sage\_fin\_full & 616 & 100.0\% & 0/587 & 0.0\% \\
\bottomrule
\end{tabular}

